DiffFNO: Diffusion Fourier Neural Operator

We introduce DiffFNO, a novel diffusion framework for arbitrary-scale super-resolution strengthened by a Weighted Fourier Neural Operator (WFNO). Mode Rebalancing in WFNO effectively captures critical frequency components, significantly improving the reconstruction of high-frequency image details that are crucial for super-resolution tasks. Gated Fusion Mechanism (GFM) adaptively complements WFNO's spectral features with spatial features from an Attention-based Neural Operator (AttnNO). This enhances the network's capability to capture both global structures and local details. Adaptive Time-Step (ATS) ODE solver, a deterministic sampling strategy, accelerates inference without sacrificing output quality by dynamically adjusting integration step sizes ATS. Extensive experiments demonstrate that DiffFNO achieves state-of-the-art (SOTA) results, outperforming existing methods across various scaling factors by a margin of 2-4 dB in PSNR, including those beyond the training distribution. It also achieves this at lower inference time. Our approach sets a new standard in super-resolution, delivering both superior accuracy and computational efficiency.

==> sec/Figures-and-Tables/Inference-Time.tex <==
\begin{table}[t]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=\linewidth, height=6.5cm, % Increased height to better fill space
            xlabel={Inference Time (ms)},
            ylabel={PSNR (dB)},
            xlabel near ticks, % Brings the label closer to the x-axis
            ylabel near ticks, % Brings the label closer to the y-axis
            ymin=28, ymax=31, % Adjusts y-axis range for tighter fit
            xmin=130, xmax=265, % Adjusts x-axis range to include all labels
            enlargelimits=0.05, % Adds a small margin to avoid label clipping
            grid=both,
            scaled ticks=false,
            clip=false,
        ]

        % DiffFNO (Ours) with red star marker
        \addplot[red, mark=star, mark size=3pt] coordinates {(141, 30.88)};
        \node[right] at (axis cs:141, 30.88) {\textbf{DiffFNO (Ours)}};

        % Other models with blue dot markers
        \addplot[blue, only marks, mark=*] coordinates {(225, 29.31)};
        \node[above] at (axis cs:225, 29.31) {LIIF \cite{SR-LIIF}};

        \addplot[blue, only marks, mark=*] coordinates {(210, 28.79)};
        \node[above] at (axis cs:210, 28.79) {LTE \cite{SR-LTE}};

        \addplot[blue, only marks, mark=*] coordinates {(240, 29.70)};
        \node[above] at (axis cs:240, 29.70) {LIT \cite{SR-LIT}};

        \addplot[blue, only marks, mark=*] coordinates {(232, 30.40)};
        \node[below] at (axis cs:232, 30.40) {LMI \cite{SR-LMI}};

        \addplot[blue, only marks, mark=*] coordinates {(248, 30.46)};
        \node[above] at (axis cs:248, 30.46) {HiNOTE \cite{SR-HiNOTE}};

        \addplot[blue, only marks, mark=*] coordinates {(195, 28.23)};
        \node[above] at (axis cs:195, 28.23) {Meta-SR \cite{SR-Meta-SR}};

        \addplot[blue, only marks, mark=*] coordinates {(147, 30.05)};
        \node[above] at (axis cs:147, 30.05) {SRNO \cite{SR-SRNO}};

        \end{axis}
    \end{tikzpicture}
    \caption{PSNR and inference time comparison for $\times$4 super-resolution. All models use the EDSR-baseline \cite{EDSR} encoder, except HiNOTE \cite{SR-HiNOTE} which has its own.}
    \label{fig:psnr_vs_inference_time}
\end{table}


==> sec/Figures-and-Tables/MERGE_Inference-Time_beside_SRNO-vs-DiffFNO.tex <==
% 双图
\twocolumn[{
\maketitle
\begin{center}
    \captionsetup{type=figure}
    \includegraphics[width=.4\textwidth]{example-image}
    \includegraphics[width=.4\textwidth]{example-image}
    \captionof{figure}{Right: PSNR and inference time comparison for $\times$4 super-resolution. All models use the EDSR-baseline \cite{EDSR} encoder, except HiNOTE \cite{SR-HiNOTE} which has its own.}
\end{center}
}]

==> sec/Figures-and-Tables/SRNO-vs-DiffFNO.tex <==
\begin{figure}[t]  % Use single-column 'figure'
  \centering
    \includegraphics[width=\columnwidth,keepaspectratio]{sec/figures/DiffFNO-vs-SRNO-2.pdf}  % Scale image to fill the column width
    \caption{Compared to SRNO \cite{SR-SRNO}, \MethodShort is strengthened by the fusion of spectral and spatial features and efficiently refined by a diffusion process.}
    \label{fig:DiffFNO-vs-SRNO}
    \vspace{-0.4cm}
\end{figure}
